Towards Seamless Management of AI Models in High-Performance Computing

With the increasing prevalence of artificial intelligence (AI) in diverse science/engineering communities, AI models emerge on an unprecedented scale among various domains. However, given the complexity and diversity of the software and hardware environments, reusing AI artifacts (models and datasets) is extremely challenging, especially with AI-driven science applications. Building an ecosystem to run and reuse AI applications/datasets at scale efficiently becomes increasingly essential for diverse science and engineering and high-performance computing (HPC) communities. In this paper, we innovate over an HPC-AI ecosystem -- HPCFair, which enables the Findable, Accessible, Interoperable, and Reproducible (FAIR) principles. HPCFair enables the collection of AI models/datasets allowing users to download/upload AI artifacts with authentications. Most importantly, our proposed framework provides user-friendly APIs for users to easily run inference jobs and customize AI artifacts to their tasks as needed. Our results show that, with HPCFair API, users irrespective of technical expertise in AI, can easily leverage AI artifacts to their tasks with minimal effort.

==> content/figtex/f00_tranfer_overview.tex <==
\begin{figure}
% \vskip 0.2in
\begin{center}

\centerline{\includegraphics[width=1.0\columnwidth]{content/figures/transfer_overview.png}

}
\caption{Why AI model knowledge matters?}
 
\label{fig:knowledge}
\end{center}
% \vskip -0.2in
\end{figure}

==> content/figtex/f02_ov_transfer.tex <==
\begin{figure}
% \vskip 0.2in
\begin{center}

\centerline{\includegraphics[width=1.0\columnwidth]{content/figures/transferAPI.pdf}

}
\caption{Overview. \ding{202} Users search target model use tag-based search. \ding{203} Load search results from HPCFair ontology and return back to users. \ding{204} Check the search results, if matches user demand fetch the target model form ontology~(as red arrow shows). If not, go \ding{205}. User choose a most relevant target model, and input the metadata and local dataset to the Knowledge transfer learning API. \ding{206} Knowledge transfer learning API fetch the target model from ontology. \ding{207} perform knowledge transfer learning and return target model container to users.}
 
\label{fig:tl}
\end{center}
% \vskip -0.2in
\end{figure}
